First measurement of elastic, inelastic and total cross-section at $\sqrt{s}=13$ TeV by TOTEM and overview of cross-section data at LHC energies

The TOTEM collaboration has measured the proton-proton total cross section at $\sqrt{s}=13$ TeV with a luminosity-independent method. Using dedicated $\beta^{*}=90$ m beam optics, the Roman Pots were inserted very close to the beam. The inelastic scattering rate has been measured by the T1 and T2 telescopes during the same LHC fill. After applying the optical theorem the total proton-proton cross section is $\sigma_{\rm tot}=(110.6 \pm 3.4$) mb, well in agreement with the extrapolation from lower energies. This method also allows one to derive the luminosity-independent elastic and inelastic cross sections: $\sigma_{\rm el} = (31.0 \pm 1.7)$ mb and $\sigma_{\rm inel} = (79.5 \pm 1.8)$ mb.

==> authorlist_cern.tex <==
%----------------------------------------------------------------------------------------------------
% Add an author
% USAGE: \AddAuthor{name}{primary affiliation}{secondary affiliation}{external affiliation}

\newif\ifFirstAuthor
\FirstAuthortrue

\def\AddAuthor#1#2#3#4{%
	\def\PriAf{#2}%
	\def\SecAf{#3}%
	\def\ExtAf{#4}%
	\def\empty{}%
	%
	\ifFirstAuthor
		\FirstAuthorfalse
	\else
		,
	\fi
	%
	\ifx\PriAf\empty
		% no primary affiliation, only external
		#1\Aref{#4}%
	\else
		\ifx\SecAf\empty
			\ifx\ExtAf\empty
				% only primary affiliation
				#1\Iref{#2}%
			\else
				% primary and external affiliation
				#1\IAref{#2}{#4}%
			\fi
		\else
			\ifx\ExtAf\empty
				% primary and secondary affiliation
				#1\IIref{#2}{#3}%
			\else
				% primary, secondary and external affiliation
				#1\IIAref{#2}{#3}{#4}%
				\relax
			\fi
		\fi
	\fi
}

%----------------------------------------------------------------------------------------------------
% Add an author
% USAGE: \AddCorrespondingAuthor{name}{primary affiliation}{secondary affiliation}{external affiliation}{footnote text}{email}

\def\AddCorrespondingAuthor#1#2#3#4#5#6{%
	\AddAuthor{#1}{#2}{#3}{*}%
	\Anotfoot{*}{#5 E-mail address: #6.}
}

%----------------------------------------------------------------------------------------------------
% Add a TOTEM institute
% USAGE: \AddInstitute{reference as in AddAuthor}{address}

\def\AddInstitute#1#2{%
	\expandafter\write1{\string\newlabel{#1}{{#1}{}}}%
	\hbox to\hsize{\strut\hss$^{#1}$#2\hss}%
}

%----------------------------------------------------------------------------------------------------
% Add an institute not in the TOTEM collaboration
% USAGE: \AddExternalInstitute{reference as in AddAuthor}{address}

\def\AddExternalInstitute#1#2{%
	\Anotfoot{#1}{#2}%
}

%----------------------------------------------------------------------------------------------------
%----------------------------------------------------------------------------------------------------
% include the actual data

\input authorlist_data

\begin{Authlist}
	\DeclareAuthors
\end{Authlist}

\DeclareInstitutes
\hbox to\hsize{\strut\hss} % trick to make institute list stop on the front page
\DeclareExternalInstitutes

